Minimizing Multimodular Functions and Allocating Capacity in Bike-Sharing Systems

The growing popularity of bike-sharing systems around the world has motivated recent attention to models and algorithms for their effective operation. Most of this literature focuses on their daily operation for managing asymmetric demand. In this work, we consider the more strategic question of how to (re-)allocate dock-capacity in such systems. We develop mathematical formulations for variations of this problem (either for service performance over the course of one day or for a long-run-average) and exhibit discrete convex properties in associated optimization problems. This allows us to design a practically fast polynomial-time allocation algorithm to compute an optimal solution for this problem, which can also handle practically motivated constraints, such as a limit on the number of docks moved in the system. We apply our algorithm to data sets from Boston, New York City, and Chicago to investigate how different dock allocations can yield better service in these systems. Recommendations based on our analysis have led to changes in the system design in Chicago and New York City. Beyond optimizing for improved quality of service through better allocations, our results also provide a metric to compare the impact of strategically reallocating docks and the rebalancing of bikes.

==> analysis_w_false_lemma.tex <==
%WE SHOULD BE A BIT MORE HIGH-LEVEL: We prove that the allocation algorithm is optimal for the operational constraints by showing that in $z$ iterations it finds the best allocation obtainable by moving at most $z$ docks within the system. This also proves a bound on the running-time,  We first define the set of feasible solutions with respect to the operational constraints.


In this section, we show that the allocation algorithm is optimal for the operational constraints introduced in Section \ref{sec: model} by proving that in $z$ iterations it finds the best allocation obtainable by moving at most $z$ docks. We thereby also provide an upper bound on the running-time of the algorithm, since any two feasible dock-allocations can be at most $D+B$ dock-moves apart. 
We begin by first formally defining the set of feasible solutions with respect to the operational constraints.
\begin{definition}
Define the $z$-\emph{ball} $S_z(\vec{d},\vec{b})$ around $(\vec{d},\vec{b})$ as the set of allocations with dock-move distance at most $2z$, %can be reached from $(\vec{d},\vec{b})$ via at most $z$ dock-moves
i.e., $S_0(\vec{d},\vec{b})=\{(\vec{d},\vec{b})\}$ and
\[
S_z(\vec{d},\vec{b}) = S_{z-1}(\vec{d},\vec{b})\cup \big( \bigcup_{(\vec{d}',\vec{b}')\in S_{z-1}(\vec{d},\vec{b})}N(\vec{d}',\vec{b}')\} \big).
\]
\end{definition}

We now want to prove that Lemma \ref{lemma: neighborhoods} continues to hold in the constrained setting; in particular, we show that with the operational constraints as well, local optima are global optima.

\begin{lemma}\label{lemma: kneighborhoods}
With $(\vec{d^+},\vec{b^+}) \in S_z(\vec{d},\vec{b})\setminus S_{z-1}(\vec{d},\vec{b})$ bike-optimal and $c(\vec{d}^\star,\vec{b}^\star)<c(\vec{d^+},\vec{b^+})$ for some $(\vec{d}^\star,\vec{b}^\star)\in S_z(\vec{d},\vec{b})\setminus S_{z-1}(\vec{d},\vec{b})$, there exists $(\vec{d}',\vec{b}')\in S_z(\vec{d},\vec{b})\cap N(\vec{d^+},\vec{b^+})$ such that 
$c(\vec{d}',\vec{b}')< c(\vec{d^+},\vec{b^+}) $. 
\end{lemma}

%\begin{proof}
\emph{Proof.} Notice that this lemma closely resembles Lemma \ref{lemma: neighborhoods}: the sole difference lies in Lemma \ref{lemma: neighborhoods} not enforcing the dock-move to maintain a bound on the distance to some allocation $(\vec{d},\vec{b})$. 

Define $(\vec{d}^\star,\vec{b}^\star)$ as in Lemma \ref{lemma: neighborhoods} with the additional restriction that $(\vec{d}^\star,\vec{b}^\star)$ be in $S_z(\vec{d},\vec{b})$, i.e., pick a solution in $S_z(\vec{d},\vec{b})$ that minimizes the dock-move distance to $(\vec{d^+},\vec{b^+})$ among solutions with strictly smaller objective value. We argue again that bike-optimality of $(\vec{d^+},\vec{b^+})$ implies that there exist $j$ and $k$, such that $d^+_j+b^+_j<d_j^\star+b_j^\star$, and $d^+_k+b^+_k>d_k^\star+b_k^\star$. Further, for any such $j$ and $k$, we can apply the proof of Lemma \ref{lemma: neighborhoods} to find a move involving at least one of the two that decreases both the objective value and the dock-move distance to $(\vec{d}^\star,\vec{b}^\star)$. 

We aim to find $j$ and $k$ such that the move identified, say from $\ell$ to $m$, is guaranteed to remain within $S_z(\vec{d},\vec{b})$.
Notice that $|\{j\}\cap\{m\}|+|\{k\}\cap\{\ell\}|\geq 1$. We know that $d_m^\star+b_m^\star>d^+_m+b^+_m$ and $d_\ell^\star+b_\ell^\star<d^+_\ell+b^+_\ell$. Suppose the move from $\ell$ to $m$ yields a solution outside of $S_z(\vec{d},\vec{b})$. It follows that $d^+_m+b^+_m\geq d_m+b_m$ and $d^+_\ell+b^+_\ell\leq d_\ell+b_\ell$, so in particular either $d^+_j+b^+_j\geq d_j+b_j$ or $d^+_k+b^+_k\leq d_k+b_k$. Thus, if we can identify $j$ and $k$ such that those two inequalities do not hold, we are guaranteed that the identified move remains within $S_z(\vec{d},\vec{b})$.
Define
%\begin{eqnarray*}
$k:=\arg\max_i\{d^+_i+b^+_i-\max\{d_i+b_i,d_i^\star+b_i^\star\}\}.$ %\end{eqnarray*}
We can then write
\vspace{-.15in}
\begin{eqnarray*}
\max_i\big\{d^+_i+b^+_i-\max\{d_i+b_i,d_i^\star+b_i^\star\}\big\}&\geq
\min_i\big\{1,\max_{i:d^+_i+b^+_i>d_i+b_i}\{(d^+_i+b^+_i)-(d_i^\star+b_i^\star)\}\big\}.
\end{eqnarray*}
\vspace{-.45in}

\noindent The minimum is at least 1 unless it is the case for all $i$ that if $d^+_i+b^+_i>d_i+b_i$ then $d^+_i+b^+_i\leq d_i^\star+b_i^\star$.
Thus, unless the above condition fails, we have identified a $k$ with the required properties. 
Suppose the condition does fail. Then $\sum_i d_i+b_i = \sum_i d_i^\star+b_i^\star = \sum_i  d^+_i+b^+_i$ and
\vspace{-.15in}
\begin{eqnarray*}
2z = \sum_i |(d_i+b_i)-(d_i^\star+b_i^\star)|=\sum_i |(d_i+b_i)-(d^+_i+b^+_i)|
\end{eqnarray*}
\vspace{-.45in}

\noindent imply that for all $i$ with $\max\{d^+_i+b^+_i,d_i^\star+b_i^\star\}>d_i+b_i$, we have $d^+_i+b^+_i=d_i^\star+b_i^\star$. Thus, it must be the case that $m$ fulfills $d^+_m+b^+_m< d_m+b_m$. 
The argument for $j$ is symmetric.\qed
%\end{proof}

By Lemma \ref{lemma: kneighborhoods}, it suffices to show that the solution found in the $z$th iteration is locally optimal among solutions in $S_{z}(\vec{d},\vec{b})$ to prove the following theorem.

%HOW ARE WE GOING TO USE THE LEMMA IN THE PROOF OF THE THEOREM: by showing that the  (which requires going through possible cases, analogue of Lemma 3).

\begin{theorem}\label{thm: koptimal}
Starting with a bike-optimal allocation $(\vec{d},\vec{b})$, in the $z$-th iteration, the discrete gradient-descent algorithm finds an optimal allocation among those in $S_z(\vec{d},\vec{b})$. Hence, the discrete gradient-descent algorithm terminates in at most $D+B$ iterations.
\end{theorem}
\emph{Proof. } We prove the theorem by induction on $z$. The base-case $z=0$ holds trivially. Suppose in the $z$th iteration, the discrete gradient-descent algorithm has found the allocation $(\vec{d}^z,\vec{b}^z) \in \arg\min_{(\vec{d}^\star,\vec{b}^\star)\in S_z(\vec{d},\vec{b})} c(\vec{d}^\star,\vec{b}^\star)$. We need to show that $(\vec{d}^{z+1},\vec{b}^{z+1})$ minimizes the objective among solutions in $S_{z+1}(\vec{d},\vec{b})$, where
%\vspace{-.25in}

\[(\vec{d}^{z+1},\vec{b}^{z+1}):=\arg\min_{(\vec{d}^{z+1},\vec{b}^{z+1})\in N(\vec{d}^z,\vec{b}^z))}\{c(\vec{d}^{z+1},\vec{b}^{z+1})\}.
\]

We first observe that by Lemma \ref{lemma: kneighborhoods}, it suffices to show that there is no better solution in $S_{z+1}(\vec{d},\vec{b})$ that is just one dock-move away from $(\vec{d}^{z+1},\vec{b}^{z+1})$. Further, by Lemma \ref{lemma: bike_opt} and the choice of dock-moves in the greedy algorithm we know that $(\vec{d}^{z+1},\vec{b}^{z+1})$ must be bike-optimal. Let $i$ be the station from which a dock was moved and let $j$ be the station to which it was moved in the $z+1$st iteration. We denote a third station by $h$ if the $z+1$st move involved a third one (recall that a dock-move from $i$ to $j$ can take an additional bike from $i$ to a third station $h$ or take one from $h$ to $j$). We can then immediately exclude the following cases:
\begin{enumerate}
\item Any dock-move in which $i$ receives a dock from some station $\ell$, including possibly $\ell=j$ or $\ell=h$, can be excluded since the greedy algorithm could have chosen to take a dock from $\ell$ instead of $i$ and found a bike-optimal allocation (by Lemma \ref{lemma: bike_opt}).
\item The same holds for any dock-move in which a dock is taken from $j$.
\item A dock-move not involving either of $i$, $j$, and $h$  yields the same improvement as it would have prior to the $z+1$st iteration. Furthermore, if such a dock-move yields a solution within $S_{z+1}(\vec{d},\vec{b})$, then prior to the $z+1$st iteration it would have yielded a solution within $S_{z}(\vec{d},\vec{b})$. Hence, by the induction assumption, it cannot yield any improvement.
\item A dock-move from station $i$ (or to $j$), as is implied by inequalities (4). (5), and (6) in the definition of multimodularity increases the objective at $i$ more (decreases the objective at $j$ less) than it would have prior to the $z+1$st iteration.
\end{enumerate}
We are left with dock-moves either from or to $h$ as well as dock-moves that involve one of the three stations only via a bike being moved. We discuss these in Appendix \ref{appendix_proof_kopt}.

%A bound on the number of iterations the greedy algorithm may run for follows immediately.

%\vspace{-.1in}

% \begin{corollary}
% The greedy algorithm terminates in at most $\sum_i d_i+b_i$ iterations.
% \end{corollary}

%In the next section we strengthen this result by using a \emph{scaling} technique.


==> model.tex <==
%\vspace{-.1in}

\input{model_new.tex}


In this section we formally define our model and discuss and justify its underlying assumptions. We begin by giving a formal definition of Raviv and Kolka's user dissatisfaction function.

\noindent\textbf{User Dissatisfaction Function}
Denote by $X=(X_1,\ldots,X_s)\in\{\pm 1\}^s$ a sequence of $s$ customers at a bike-share station. The sign of $X_t$ identifies whether customer $t$ arrives to rent ($X_t=-1$) or to return a bike ($X_t=1$). We take this sequence as {\em exogenously} given, even though in reality it depends on capacity decisions. We will explore and justify this modeling choice in detail below.
The truncated sequence $(X_1,\ldots,X_t)$ is written as $X(t)$. We denote throughout by $d$ and $b$ the number of open docks and available bikes at a station before any customer has arrived. A station with $d$ open docks and $b$ available bikes has $d+b$ docks in total.
Whenever a customer arrives to return a bike at a station and there is an open dock, the customer returns the bike, the number of available bikes increases by 1, and the number of open docks decreases by 1. Similarly, a customer arriving to rent a bike when one is available decreases the number of available bikes by 1 and increases the number of open docks by 1.
If instead a customer arrives to rent (return) a bike when no bike (open dock) is available, then she disappears with an out-of-stock event. We assume that only customers affect the inventory-level at a station, i.e., no rebalancing occurs. It is useful then to write 

\vspace{-.5in}

\begin{eqnarray*}
\delta_{X(t)}(d,b):=\max\{0,\min\{d+b,\delta_{X(t-1)}-X_t\}\},\; \delta_{X(0)}(d,b)=d \\
\beta_{X(t)}(d,b):=\max\{0,\min\{d+b,\beta_{X(t-1)}+X_t\}\}, \; \beta_{X(0)}(d,b)=b
\end{eqnarray*}

\vspace{-.2in}

\noindent as a shorthand for the number of open docks and available bikes after the first $t$ customers. \dfedit{Notice that the arrival of a customer only affects the number of bikes in the station, but not the total number of docks at the station, i.e., $\delta_{X(t)}(d,b)+\beta_{X(t)}(d,b)=d+b\;\forall t$.}

%I WRITE "THEN" A LOT, MAYBE TOO MUCH

Our objective is based on the number of out-of-stock events. In accordance with the above-described model, customer $t$ experiences an out-of-stock event if and only if $\delta_{X(t)}(d,b)=\delta_{X(t-1)}(d,b)$, that is, out-of-stock events occur if and only if an arriving customer does not change the number of bikes at the station. Since $d+b= \delta_{X(t)}(d,b)+\beta_{X(t)}(d,b)$ for every $t$, this happens if and only if $\beta_{X(t)}(d,b)=\beta_{X(t-1)}(d,b)$. Since we are interested in the number of out-of-stock events as a function of the initial number of open docks and available bikes, we can write our cost-function as
$c^{X}(d,b)=|\{\tau: X_\tau=1, \delta_{X(\tau-1)}(d,b)=0 \}|+|\{\tau: X_\tau=-1, \beta_{X(\tau-1)}(d,b)=0 \}|.$ 
%\vspace{-.1in}
%\noindent 
% \authorsdelete{Starting with $c^{X(0)}(d,b)=0$, $c^{X(t)}(d,b)$ then fulfills the recursion
% %\vspace{-.1in}
% %\begin{eqnarray*}
% $c^{X(t)}(d,b)=c^{X(t-1)}(d,b)+\mathbf{1}_{\{\beta_{X(t)}(d,b)=\beta_{X(t-1)}(d,b)\}}$.}
% %\end{eqnarray*}

\OneAndAHalfSpacedXI
\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.6\textwidth]{Figures/Fig_2a.jpg}
  \caption{As a function of bikes for stations with capacity~39.}
  \label{fig:4UDFs}
\end{subfigure}%
\begin{subfigure}{.555\textwidth}
  \centering
  \includegraphics[width=.633\textwidth]{Figures/Fig_2b.jpg}
  \caption{As a function of $(d,b)$ at a single station.}
  \label{fig:sub2}
\end{subfigure}
\caption{Visualizations of user dissatisfaction functions based on real data.}
\label{fig:UDF2D}
\end{figure}
\DoubleSpacedXI

%\vspace{-.1in}

\noindent\textbf{Optimization Problem}
Given for each station $i\in[n]:=\{1,2,\ldots,n\}$ a distribution $p_i$ over possible sequences of arrivals $\{(\pm 1)^s, s\in\mathbb{N}_0\}$, which we call the \emph{demand-profile}, we can write $c_i(d,b)=\mathbb{E}_{X\sim p_i}[c^X(d,b)]$ for the expected number of out-of-stock events at station~$i$ and $c(\vec{d},\vec{b})=\sum_i c_i(d_i,b_i)$. Figure \ref{fig:4UDFs} shows the user dissatisfaction functions at three different stations for a fixed number of docks and varying number of bikes; Figure \ref{fig:sub2} indicates for a single station how its UDF changes with varying capacity.
We then want to solve, given budgets $B$ on the number of bikes and $D+B$ on the number of docks, a current allocation $(\vec{\bar{d}},\vec{\bar{b}})$, a constraint $z$ on the number of docks moved, and lower/upper bounds $l_i,u_i$ for each station $i$, the following minimization problem
%We then want to solve, for parametersD,B, (~ ̄d,~ ̄b), andz, as well asli,uifor eachi∈[n], the following minimization problem
\OneAndAHalfSpacedXI
\begin{equation*}
\begin{aligned}
\mathtt{minimize}_{(\vec{d},\vec{b})} & c(\vec{d},\vec{b})\\
s.t. &  \sum_i d_i+b_i &\leq D+B,\\
& \sum_i b_i & \leq B, \\
&\sum_i |(\bar{d}_i+\bar{b}_i)-(d_i+b_i)|& \leq 2z,\\
\forall i\in[n]: & l_i\leq \; d_i+b_i &\leq u_i.
\end{aligned}
\tag{P1}\label{opt:original}
\end{equation*}
\DoubleSpacedXI

%\vspace{-.25in}

Here, the first constraint corresponds to a budget on the number of docks, the second to a budget on the number of bikes, the third to the operational constraints and the fourth to the lower and upper bounds on the number of docks at each station; for notational convenience it will be simpler to assume that $c_i(d_i,b_i)=\infty$ if $d_i+b_i>u_i$ or $d_i+b_i<l_i$. \dfedit{Then the last row of inequalities in \ref{opt:original} can be dropped, as the objective evaluates to infinity when it is violated. 
%Next, observe that since $c_i(d,b)$ is non-increasing in both arguments while $d_i+b_i<u_i$, we know that unless $\sum_i u_i < D+B$, the optimal solution fulfills $\sum_i d_i+b_i=D+B$, implying that the first constraint holds with equality.\footnote{This assumes that $\sum_i \bar{d}_i+\bar{b}_i=D+B$, i.e., the problem is only about reallocating existing capacity; if there exists additional capacity, then .}
In addition, we may add a dummy (``depot'') station $\mathcal{D}$ that observes no demand, i.e., with $c_\mathcal{D}(d,b)=0$ if $l_\mathcal{D}\leq d+b\leq u_\mathcal{D}$, and $c_\mathcal{D}(d,b)=\infty$ otherwise, to guarantee that the first two constraints hold with equality. Thus, we can transform our original optimization problem into one of the following form, which is our focus throughout the main body of the text:
\OneAndAHalfSpacedXI
\begin{equation*}
\begin{aligned}
\mathtt{minimize}_{(\vec{d},\vec{b})} & c(\vec{d},\vec{b})\\
s.t. &  \sum_i d_i+b_i &= D+B,\\
& \sum_i b_i & = B, \\
&\sum_i |(\bar{d}_i+\bar{b}_i)-(d_i+b_i)|& \leq 2z.
\end{aligned}
\tag{P2}\label{opt:adapted}
\end{equation*}
\DoubleSpacedXI
We defer the details around how to use $\mathcal{D}$ to transform \ref{opt:original} into \ref{opt:adapted} to Appendix \ref{appendix:tradeoff}. There, we also show how to optimally solve an optimization problem that involves an additional trade-off between the size of $D$ and the size of $z$, i.e., between the costs of additional docks and \dfedit{the cost of} moving docks.}


% Optimizing with a dock budget of $D+2B$, a solution to the optimization problem with $d_i^\star$ empty docks and $b_i^\star$ full docks at each station $i$ is then equivalent (in objective) to a solution to the second optimization problem with  $b_\mathcal{D}=B-\sum_i b_i^\star, d_\mathcal{D}=\sum_ib_i^\star$, and $d_i=d_i^\star, b_i=b_i^\star$ for all other $i$. This allows us to turn the second inequality of the optimization problem into an equality.
%
%we then run the algorithm with a dock-budget of $D+2B$, we are guaranteed that both constraints hold with equality since all excess bikes and docks can be placed at~$\mathcal{D}$. In particular, for any solution that does not use all $B$ bikes and $D+B$ docks in the original problem, there exists an equivalent solution in the problem with $\mathcal{D}$ and dock budget $D+2B$ where the excess bikes/docks are at $\mathcal{D}$, the constraints hold with equality, and the objective is the same. Here, $D$ may include docks that are currently part of the system as well as inventory that is meant to be added to the system. 

% In fact, in Appendix 
%to ensure that, % \dfedit{. For the first constraint this holds true because $c(\cdot,\cdot)$ is non-increasing in both arguments. To ensure that the second constraint holds with equality}, 

%Also, we may assume that $\sum_i (\bar{d}_i+\bar{b}_i=D+B$ even if there are docks at our disposal beyond the ones currently in operation --- to do so we add a dummy station, also with cost 0, that holds the additional docks in $(\vec{\bar{d}},\vec{\bar{b}})$.

% \OneAndAHalfSpacedXI
% \dfedit{
% \addtolength{\tabcolsep}{3pt}    
% \begin{table}[ht]
% \centering
% \begin{tabular}{l|l|l|}
% \hline
% \multicolumn{1}{|c|}{Dock} & & $d_i$ or $b_i$ \\
% \multicolumn{1}{|c|}{empty dock} & & $d_i$ or $b_i$ \\
% \hline
% %\multicolumn{1}{|c|}{Boston}        &           &            &               \\ \hline
% \end{tabular}
% \caption{{Glossary of bike-sharing terms and their mathematical translation.}}
% \label{table: glossary}
% \end{table}
% \addtolength{\tabcolsep}{-3pt}    
% }
% \DoubleSpacedXI



%Can handle linear cost at each location, in practice, assuming costs are uniform is appropriate given that (i) administrative effort dominates maintenance effort, (ii) requires stakeholders' approval.




==> scaling.tex <==
% !TEX root = main.tex

We now extend our analysis in Section \ref{sec: kstepopt} to adapt our algorithm to a scaling algorithm that provably finds the optimal allocation of bikes and docks in~$O\big(n\log(B+D)\big)$ iterations. The idea underlying the scaling algorithm is to first find the optimal allocation of bikes and docks with each $d_i$ and each $b_i$ being a multiple of $2^{k+1}$ (for a fixed $k$). From this allocation, we can show how to extend our previous gradient-descent analysis to guarantee that we can find, in $O(n)$ iterations, an allocation that is optimal subject to each $d_i$ and each $b_i$ equal to a multiple of $2^{k}$. Repeating this process $\lfloor\log_2(B+D) \rfloor+1$ times we find the optimal allocation in which each $d_i$ and each $b_i$ is a multiple of~$2^0=1$, i.e., the optimal allocation.

 Notice first that if $f(d,b)$ is multimodular, then $f(\alpha d, \alpha b)$ is as well for any integer $\alpha\geq 0$. Thus, we can adapt the greedy algorithm to move $\alpha$ empty/full docks or $\alpha$ bikes, instead of one, in any move; the analysis in the last two sections guarantees that such an algorithm finds the optimal allocation of bikes and docks in which each $d_i$ and each $b_i$ is a multiple of $\alpha$ in at most $(D+B)/\alpha$ dock moves. What remains to be shown is a bound on the number of moves needed (each moving $2^k$ docks/bikes) from a solution $(\vec{d}^{k+1},\vec{b}^{k+1})$ that is optimal subject to the additional constraint that each $d_i^{k+1}$ and each $b_i^{k+1}$ a multiple of $2^{k+1}$ to a solution $(\vec{d}^{k},\vec{b}^{k})$ that is optimal subject to the weaker constraint that each $d_i^k$ and each $b_i^k$ is a multiple of $2^{k}$.
 
 \begin{lemma}
 Let $(\vec{d}',\vec{b}')$ be the allocation of bikes and docks that has the same allocation of docks as $(\vec{d}^{k+1},\vec{b}^{k+1})$, but has an optimal allocation of bikes subject to the constraint that each station has a multiple of $2^k$ bikes allocated to it. If $(\vec{d}^{k},\vec{b}^{k})$ is the solution with minimum dock-move distance to $(\vec{d}',\vec{b}')$ in addition to its constraints above, then that dock-move distance is bounded by 12$n$.
 \end{lemma}
 
 \emph{Proof Sketch.} Suppose first it was the case that $(\vec{d}^{k+1},\vec{b}^{k+1})=(\vec{d}',\vec{b}')$. Then the idea of the proof is as follows: we know that doing the same move (each one moving $2^k$ docks/bikes) twice when starting from $(\vec{d}^{k+1},\vec{b}^{k+1})$ cannot yield improvement by definition of $(\vec{d}^{k+1},\vec{b}^{k+1})$. Consider an allocation obtained by doing all but two of the moves the greedy algorithm takes to go from $(\vec{d}',\vec{b}')$ to $(\vec{d}^{k},\vec{b}^{k})$. By the optimality of $(\vec{d}^{k},\vec{b}^{k})$, doing the two moves yields improvement (when only two moves away from $(\vec{d}^{k},\vec{b}^{k})$), but by multimodularity (follows from the same inequalities as in Theorem \ref{thm: koptimal}) they yield at least as much improvement when carried out from $(\vec{d}',\vec{b}')$. Thus, for example it cannot be the case that the greedy algorithm twice takes an empty dock from $i$ and twice gives an empty dock to $j$ along its path. But then, each of the four possible moves can appear at most $n$ times since otherwise, by the pigeonhole principle, there would be two occurrences of the same move at a station.\footnote{Notice that it may not be the same move that appears twice, e.g., it could be the case that $e_{ij}$, $e_{kj}$ and $e_{i\ell}$ occur, but these are equivalent to $e_{ij},e_{ij}$, and $e_{k\ell}$.} This bounds the distance by $4n$ in the case that $(\vec{d}^{k+1},\vec{b}^{k+1})=(\vec{d}',\vec{b}')$.
 
 A similar idea works when $(\vec{d}^{k+1},\vec{b}^{k+1})\neq(\vec{d}',\vec{b}')$, but requires a few additional insights. Notice first that $\sum_i|b^{k+1}_i-b'_i|$ is bounded by $2n$ by definition of $(\vec{d}^{k+1},\vec{b}^{k+1})$ (else, moving two bikes would yield improvement). For each station $i$, let $x_i:=b^{k+1}_i-b'_i$. If $x_i<0$, then $2^k$ additional bikes/full docks at $i$ yield greater improvement in  $(\vec{d}^{k+1},\vec{b}^{k+1})$ than in $(\vec{d}',\vec{b}')$ and taking $2^k$ empty docks has smaller cost. On the other hand, taking $2^k$ bikes/full docks has greater cost and adding $2^k$ empty docks yields smaller improvement in $(\vec{d}^{k+1},\vec{b}^{k+1})$ than in $(\vec{d}',\vec{b}')$. The reverse is true when $x_i>0$. However, using the multimodular inequalities we observe that doing these changes for the $x$th time at $(\vec{d}',\vec{b}')$ yields smaller improvement (greater cost) than it does for the first time at $(\vec{d}^{k+1},\vec{b}^{k+1})$. Thus, we can bound the number of moves when starting from $(\vec{d}',\vec{b}')$ via a bound on the moves that yield improvement from $(\vec{d}^{k+1},\vec{b}^{k+1})$. \qed
 %Thus, Further, we know that when starting the greedy algorithm from $(\vec{d}',\vec{b}')$, then (i) bike-optimality (subject to multiples of $2^k$) is preserved in each iteration, and (ii) after $\ell$ greedy moves, we have the optimal allocation of bikes and docks that can be achieved by moving at most $\ell$ times $2^k$ bikes/docks when starting from $(\vec{d}',\vec{b}')$. Suppose it took $L$ moves from $(\vec{d}',\vec{b}')$ to get to the optimum and $L>12n$. Then there must exist stations $i$ and $j$ such that (i) $i$ receives at least 2 empty docks in the $L$ moves or $i$ receives at least 2 full docks in the $L$ moves and (ii) 
 %\qed
 \begin{theorem}
 The scaling algorithm terminates in $O\big(n\log(B+D)\big)$ iterations.
 \end{theorem}

% Let $(\vec{d}^*,\vec{b}^*)$ denote the globally optimal allocation of bikes and docks and $(\vec{d},\vec{b})$ be the allocation that is optimal with the added constraint that each $d_i$ and each $b_i$ is even.

% \begin{lemma}\label{lem:bikenonopt}
% Suppose $(\vec{d}',\vec{b}')$ is not bike-optimal, but has the property that none of the four possible dock-moves improves its objective. Then there exists an optimal allocation of bikes and docks $(\vec{d}^*,\vec{b}^*)$ that allocates the same number of docks to each station, i.e. $d_i+b_i=d_i^*+b_i^*\;\forall i$.
% \end{lemma}


% \begin{lemma}
% Let $(\hat{\vec{d}},\hat{\vec{b}})$ be the allocation of bikes and docks that minimizes $c(\vec{d},\vec{b})$ among all allocations with the property that $d_i$ and $b_i$ are even for all $i$. Then there exists an allocation of bikes and docks $(\vec{d}',\vec{b}')$ that (i) fulfills the assumption of Lemma \ref{lem:bikenonopt}, and (ii) is at most $4n$ dock-moves away from $(\hat{\vec{d}},\hat{\vec{b}})$.
% \end{lemma}

% \begin{proof}
% Our proof consists of three parts. We know from Theorem \ref{thm: koptimal} that the number of dock-moves used by the algorithm is equal to the dock-move distance of interest. Consider the exact moves the algorithm performs. We first show that if we have more than $n$ moves of any one type (e.g., moving an empty dock from one station to another more than $n$ times), then there exists a path of the same length to the same allocation that involves the exact same move twice (e.g., moving two empty docks from station $i$ to $j$). Then, we show that performing these two moves (or this one move twice) when starting from $(\vec{d},\vec{b})$ yields an improvement. Finally, we note that performing these moves from $(\vec{d},\vec{b})$  yields a new solution in which the number of empty docks and the number of bikes at each station is even; this contradicts the definition of $(\vec{d},\vec{b})$ as the  the allocation that is optimal with the added constraint that each $d_i$ and each $b_i$ is even. This contradiction implies that the path from $(\vec{d},\vec{b})$ to $(\vec{d}^*,\vec{b}^*)$ contains at most $n$ moves for each of the four types which implies the statement. \qed
% \end{proof}





